Counting loop diagrams: computational complexity of higher-order amplitude evaluation

We discuss the computational complexity of the perturbative evaluation of scattering amplitudes, both by the Caravaglios-Moretti algorithm and by direct evaluation of the individual diagrams. For a self-interacting scalar theory, we determine the complexity as a function of the number of external legs. We describe a method for obtaining the number of topologically inequivalent Feynman graphs containing closed loops, and apply this to one- and two-loop amplitudes. We also compute the number of graphs weighted by their symmetry factors, thus arriving at exact and asymptotic estimates for the average symmetry factor of diagrams. We present results for the asymptotic number of diagrams up to 10 loops, and prove that the average symmetry factor approaches unity as the number of external legs becomes large.

==> figs/oneloopfig0 <==
#FIG 3.2
Landscape
Center
Metric
A4      
100.00
Single
-2
1200 2
1 3 0 2 0 0 50 0 46 0.000 1 0.0000 2700 5355 64 64 2700 5355 2745 5400
1 3 0 2 0 0 50 0 46 0.000 1 0.0000 2700 4815 64 64 2700 4815 2745 4860
1 3 0 2 0 0 50 0 46 0.000 1 0.0000 2700 4275 64 64 2700 4275 2745 4320
1 3 0 2 0 7 50 0 46 0.000 1 0.0000 6345 4950 1733 1733 6345 4950 6708 3255
2 1 0 2 0 7 50 0 46 0.000 0 0 -1 0 0 2
	 8055 4950 11160 4950
2 1 0 2 0 7 50 0 46 0.000 0 0 -1 0 0 2
	 5224 6259 2974 8824
2 1 0 2 0 7 50 0 46 0.000 0 0 -1 0 0 2
	 4711 5593 2011 6808
2 1 0 2 0 7 50 0 46 0.000 0 0 -1 0 0 2
	 4771 4229 2026 2789
2 1 0 2 0 7 50 0 46 0.000 0 0 -1 0 0 2
	 5288 3620 3083 1100
4 0 0 50 0 0 72 0.0000 4 735 405 10620 4590 1\001


==> figs/oneloopfig1 <==
#FIG 3.2
Landscape
Center
Metric
A4      
100.00
Single
-2
1200 2
1 3 0 3 0 0 50 0 41 0.000 1 0.0000 3960 4860 186 186 3960 4860 3780 4815
1 3 0 3 0 0 50 0 41 0.000 1 0.0000 3960 5625 162 162 3960 5625 3825 5535
2 1 0 3 0 0 50 0 41 0.000 0 0 -1 0 0 2
	 6300 4950 9180 4950
2 1 0 3 0 0 50 0 41 0.000 0 0 -1 0 0 2
	 6300 4950 4230 2520
2 1 0 3 0 0 50 0 41 0.000 0 0 -1 0 0 2
	 6300 4950 2475 4050
2 1 0 3 0 0 50 0 41 0.000 0 0 -1 0 0 2
	 6300 4950 3285 1440
2 1 0 3 0 0 50 0 41 0.000 0 0 -1 0 0 2
	 6255 4950 2655 6750
2 1 0 3 0 0 50 0 41 0.000 0 0 -1 0 0 2
	 6300 4950 3780 8460
4 0 0 50 0 0 80 0.0000 4 810 450 3915 1350 1\001
4 0 0 50 0 0 80 0.0000 4 825 450 2700 3825 0\001
4 0 0 50 0 0 80 0.0000 4 825 450 2340 6345 0\001
4 0 0 50 0 0 80 0.0000 4 825 450 3465 8235 0\001
4 0 0 50 0 0 80 0.0000 4 810 450 8955 4635 1\001


==> figs/oneloopfig2 <==
#FIG 3.2
Landscape
Center
Metric
A4      
100.00
Single
-2
1200 2
1 3 0 3 0 0 50 0 41 0.000 1 0.0000 3960 4860 186 186 3960 4860 3780 4815
1 3 0 3 0 0 50 0 41 0.000 1 0.0000 3960 5625 162 162 3960 5625 3825 5535
2 1 0 3 0 0 50 0 41 0.000 0 0 -1 0 0 2
	 6300 4950 9180 4950
2 1 0 3 0 0 50 0 41 0.000 0 0 -1 0 0 2
	 6300 4950 4230 2520
2 1 0 3 0 0 50 0 41 0.000 0 0 -1 0 0 2
	 6300 4950 2475 4050
2 1 0 3 0 0 50 0 41 0.000 0 0 -1 0 0 2
	 6300 4950 3285 1440
2 1 0 3 0 0 50 0 41 0.000 0 0 -1 0 0 2
	 6255 4950 2655 6750
2 1 0 3 0 0 50 0 41 0.000 0 0 -1 0 0 2
	 6300 4950 3780 8460
4 0 0 50 0 0 80 0.0000 4 825 450 2340 6345 0\001
4 0 0 50 0 0 80 0.0000 4 825 450 3465 8235 0\001
4 0 0 50 0 0 80 0.0000 4 810 450 8955 4635 1\001
4 0 0 50 0 0 80 0.0000 4 825 450 3915 1350 0\001
4 0 0 50 0 0 80 0.0000 4 810 450 2700 3825 1\001


==> figs/oneloopfig3 <==
#FIG 3.2
Landscape
Center
Metric
A4      
100.00
Single
-2
1200 2
1 3 0 3 0 7 50 0 -1 0.000 1 0.0000 6300 4950 2172 2172 6300 4950 4140 5175
1 3 0 3 0 0 50 0 41 0.000 1 0.0000 2745 4905 45 45 2745 4905 2700 4905
1 3 0 3 0 0 50 0 41 0.000 1 0.0000 2745 5445 45 45 2745 5445 2745 5400
1 3 0 3 0 0 50 0 41 0.000 1 0.0000 2745 5940 45 45 2745 5940 2700 5940
2 1 0 3 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4860 3330 2700 630
2 1 0 3 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4185 4500 1620 3825
2 1 0 3 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4365 5940 1755 7065
2 1 0 3 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5130 6795 2745 9315
2 1 0 3 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 8505 4950 11025 4950
4 0 0 50 0 0 80 0.0000 4 825 450 3915 1395 0\001
4 0 0 50 0 0 80 0.0000 4 825 450 1980 3510 0\001
4 0 0 50 0 0 80 0.0000 4 825 450 1935 6570 0\001
4 0 0 50 0 0 80 0.0000 4 825 450 2745 8955 0\001
4 0 0 50 0 0 80 0.0000 4 810 450 10305 4635 1\001

